On Mixing in Pairwise Markov Random Fields with Application to Social Networks

We consider pairwise Markov random fields which have a number of important applications in statistical physics, image processing and machine learning such as Ising model and labeling problem to name a couple. Our own motivation comes from the need to produce synthetic models for social networks with attributes. First, we give conditions for rapid mixing of the associated Glauber dynamics and consider interesting particular cases. Then, for pairwise Markov random fields with submodular energy functions we construct monotone perfect simulation.

==> 3_Efficiency.tex <==
\section{Efficiency of the result}
||||| перенести

First of all, we must notice here, that independently from temperature mixing time is at least of order $n \ln(n)$. It is so, because achieving stationary distribution by iterating means that every vertex has to be updated at least once. And with $n\to \infty$ we have to do of order $n\ln(n)$ Markov chain steps to obtain the probability of updating each vertex at least once tending to 1.

%========================================================


%\subsection{General approach}
%Now we are about to give general upper bound on mixing time, which is independent from the system temperature. Let us introduce a general theorem, which is given in [2] and adapted here for our model.
%\begin{Theorem}
%Let $$\delta_v = \sup\{| \varepsilon(\sigma) - \varepsilon(\tau)|\ :\ \forall w \in V\setminus \{v\}\to \sigma(w) = \tau(w) \},$$ and 
%$$\delta = \sup_{v \in V} \delta_v.$$
%Then
%$$ ||\pi^0 P^t - \pi||_{TV} \leq \frac{1}{2}|| \pi^0 - \pi ||_{TV}(1 - e^{-n\delta})^t.$$
%\end{Theorem}
%Now we estimate $\delta$ and then see the bound which is provided by this theorem. Let $\sigma$ and $\tau$ be two arbitrary configurations which agree everywhere but in the vertex $v$. Then
%$$| \varepsilon(\sigma) - \varepsilon(\tau) | = \left | \sum_{w \sim v}(\sigma(w) - \sigma(v))^2 - \sum_{w \sim v}(\tau(w) - \tau(v)) ^ 2 \right |  = $$
%$$ = \left|\sum_{w \sim v}\left (2\sigma(i) - \sigma(v) - \tau(v)\right )\left (\tau (v) - \sigma(v) \right)\right| =$$ 
%$$= {\sf deg}(v)\cdot|\sigma(v) - \tau(v)|\left| 2s - \sigma(v) - \tau(v) \right|,$$

%where $s = \frac{1}{{\sf deg}(v)}\sum \limits_{i \sim v}\sigma(i).$ Recall, that $\triangle$ is the maximum degree of graph. Now is easy to see, that
%$$m^2 \leq \delta \leq 2m^2 \cdot \triangle$$
%and since that, $t$ must be at least of order $e^{n \delta}$ to put inequality in theorem under the $\varepsilon$.
%So, it can be seen now, that general approach, which is about not to take temperature of the system into consideration, does not give us any significant result. 

Let us show now, that it is impossible to proof fast mixing in the way of ignoring temperature. In other words, there is a graph and a temperature, that force our Markov chain to mix in exponential time.



%\subsection{Complete graph}
Here we are about to consider configurations on the complete graph. Let $S \subset \Omega$ be the subset of the Markov chain state space $\Omega$, $S^c = \Omega \setminus S$ and for $A,B \subset \Omega$
$$ Q(A,B)  = \sum_{a\in A, b \in B}\pi(a)P_{a,b},$$
where $\pi$ is stationary distribution. We call $\Phi(S)$ the \textit{bottleneck ratio} of the set $S$ where
$$\Phi(S) = \frac{Q(S, S^c)}{\pi(S)},\ \pi(S) = \sum_{\sigma \in \Omega}\pi(\sigma)$$
and $\pi(S) < 1/2$. Then there is the following lower bound for mixing time (see [1] for details):
\begin{equation}
t_{mix}(\varepsilon) \geq \frac{\frac{1}{2} - \varepsilon}{\Phi(S)},
\end{equation}
which holds for all $S \subset \Omega$. We consider $\varepsilon$ here as constant less than a half. And since that if we are about producing exponential lower found for $t_{mix}$ all we need is to find appropriate $S$. Intuitively, $S$ must be the set of states which is hard to escape from. The following example of $S$ is not the optimal one, it is not the most narrow place of the graph, but it will be enough for our aims. Let consider $S$ like a set of just one configuration with all values equal 0, let us call this state as $\hat{0}$. Then
$$\Phi(S) = \frac{Q(S, S^c)}{\pi(S)} = \frac{\pi(\hat{0})\sum \limits_{\sigma \in \Omega \setminus {\hat{0}}}P_{\hat{0}, \sigma}}{\pi(\hat{0})} = n\left(\frac{1}{n} \sum \limits_{k = 1}^m e^{-\beta k^2(n-1)} \right ) Z^{-1}(\beta) \leq$$
$$ \leq me^{-\beta(n-1)}Z^{-1}(\beta), $$
and since $Z(\beta) > e^{-\beta \cdot 0} = 1$, then 
\begin{equation}
\Phi(S) \leq me^{-\beta(n-1)}.
\end{equation}
Hence, if, for example, $\beta = 1$ is fixed, then (8) and (9) give us exponential lower bound for mixing time. Thus, complete graph is an example which shows that sometimes it may take very long time to get close to stationary distribution.
%\subsection{Separate-edges graph}
%To cover all the cases we have to answer the question if there is a graph for which Markov chain mix fast independently of temperature. Here we consider very specific case of graph $G = (V,E)$, where $\forall v \exists! w:\{v,w\}\in E $.

==> 5_Matching.tex <==

In this section we try to fit real social networks to our model.
Towards this goal, we shall employ the maximum log-likelihood method.
The log-likelihood function for our model takes the form
$$
\log(\pi(\sigma)) = \log(e^{-\beta\varepsilon(\sigma)}) 
- \log\left(\sum_{\tau \in M^G}e^{-\beta\varepsilon(\tau)}\right)
$$
$$
=-\beta \varepsilon(\sigma) - \log\left(\sum_{\tau \in M^G}e^{-\beta\varepsilon(\tau)}\right).
$$
Now let us differentiate the above expression with respect to $\beta$.
$$
\frac{d}{d\beta} \log(\pi(\sigma)) = 
- \varepsilon(\sigma) -\frac{1}{\sum \limits_{\tau \in M^G}e^{-\beta\varepsilon(\tau)}} 
\sum \limits_{\tau \in M^G} (-\varepsilon(\tau))e^{-\beta\varepsilon(\tau)}.
$$
Equating the derived expression to zero, we obtain
$$
\sum_{\tau \in M^G} \frac{\varepsilon(\tau)e^{-\beta\varepsilon(\tau)}}{\sum_{\tau' \in M^G}e^{-\beta\varepsilon(\tau')}}
= \varepsilon(\sigma),
$$ 
or, equivalently,
$$
\sf{E}_\beta[\varepsilon(\tau)] = \varepsilon(\sigma).
$$
We can estimate the left hand side by
$$
\sf{E}_\beta[\varepsilon(\tau)] = \frac{1}{N} \sum_{k=1}^{N} \varepsilon(\tau_k),
$$
where $\tau_k$ are generated by perfect MCMC as described in the previous section.



===============================================

\subsection{Matching}

Since we can sample from \textit{general distribution}, we can try to fit real social networks to our model.
Towards this goal, we shall employ the maximum log-likelihood method.
The log-likelihood function for our model takes the form
$$
\log(\pi(\sigma)) = \log(e^{-\beta\varepsilon(\sigma)}) 
- \log\left(\sum_{\tau \in M^G}e^{-\beta\varepsilon(\tau)}\right)
$$
$$
=-\beta \varepsilon(\sigma) - \log\left(\sum_{\tau \in M^G}e^{-\beta\varepsilon(\tau)}\right).
$$
Now let us differentiate the above expression with respect to $\beta$.
$$
\frac{d}{d\beta} \log(\pi(\sigma)) = 
- \varepsilon(\sigma) -\frac{1}{\sum \limits_{\tau \in M^G}e^{-\beta\varepsilon(\tau)}} 
\sum \limits_{\tau \in M^G} (-\varepsilon(\tau))e^{-\beta\varepsilon(\tau)}.
$$
Equating the derived expression to zero, we obtain
$$
\sum_{\tau \in M^G} \frac{\varepsilon(\tau)e^{-\beta\varepsilon(\tau)}}{\sum_{\tau' \in M^G}e^{-\beta\varepsilon(\tau')}}
= \varepsilon(\sigma),
$$ 
or, equivalently,
$$
\sf{E}_\beta[\varepsilon(\tau)] = \varepsilon(\sigma).
$$
We can estimate the left hand side by
$$
{\sf E}_\beta[\varepsilon(\tau)] = \frac{1}{N} \sum_{k=1}^{N} \varepsilon(\tau_k),
$$
where $\tau_k$ are generated by perfect MCMC as described in the previous section.

